A Probabilistic Framework and a Homotopy Method for Real-time Hierarchical Freight Dispatch Decisions

We propose a real-time decision framework for multimodal freight dispatch through a system of hierarchical hubs, using a probabilistic model for transit times. Instead of assigning a fixed time to each transit, we advocate using historical records to identify characteristics of the probability density function for each transit time. We formulate a nonlinear optimization problem that defines dispatch decisions that minimize expected cost, using this probabilistic information. Finally, we propose an effective homotopy algorithm that (empirically) outperforms standard optimization algorithms on this problem by taking advantage of its structure, and we demonstrate its effectiveness on numerical examples.

==> Transportation Research copy/commondefinitions.tex <==

%-----------------Modifications to algorithm environment ----------
%\renewcommand{\algorithmicendfor}{\algorithmicend}
%\renewcommand{\algorithmicendwhile}{\algorithmicend}
%\renewcommand{\algorithmicendif}{\algorithmicend}
%\renewcommand{\algorithmicdo}{}


%--------------- Spacing -------------------------------------------

\newcommand{\newpart}{\medskip \par \noindent}
\newcommand{\opn}{\bigskip}

%---------------- Color --------------------------------------------

% Sample commands:
%     \colorbox{red}{blah.}
%     \color{red}{nnnnn}
%     {\color{blue} nisxxx}
% Hansen, Nagy, O'Leary:
%  Red:   CMYK 0441
%  Blue:  CMYK 4301
%  Green: CMYK 3042

%\definecolor{gold}{rgb}{0.85,.66,0}
\definecolor{plum}{rgb}{0.45,0,.66}
\definecolor{mythistle}{rgb}{.99,.195,.133}
%\definecolor{bgn}{rgb}{0,.85,.46}  %bluegreen
%\definecolor{ngn}{rgb}{0,1,0}  %newgreen
%\definecolor{myred}{rgb}{1,.1,.16}  %deeper red
\definecolor{myred}{cmyk}{0.000000,1.000000,1.000000,0.1}
\definecolor{myblue}{cmyk}{1.000000,0.750000,0.000000,0.1}
\definecolor{mybgn}{cmyk}{0.850000,0.350000,0.000000,0.1}
\definecolor{mygrn}{cmyk}{0.750000,0.000000,1.000000,0.2}
%\definecolor{myplum}{cmyk}{0.050000,0.250000,1.000000,0.2}
%\newcommand{\cblu}[1]{{\color{myblue}{#1}}}
\newcommand{\cblu}[1]{{\color{blue}{#1}}}
\newcommand{\cblack}[1]{{\color{black}{#1}}}
%\newcommand{\cplm}[1]{{\color{myplum}{#1}}}
\newcommand{\cred}[1]{{\color{myred}{#1}}}
\newcommand{\cyel}[1]{{\color{gold}{#1}}}
\newcommand{\cgrn}[1]{{\color{mygrn}{#1}}}
\newcommand{\cplm}[1]{{\color{plum}{#1}}}
\newcommand{\cbgn}[1]{{\color{mybgn}{#1}}}
\newcommand{\cdef}[1]{{\bf \cblu{#1}}\index{#1}}
\newcommand{\cdefno}[1]{{\bf \cblu{#1}}} % definition without index entry
\newcommand{\cemph}[1]{\cblu{#1}}
\newcommand{\cerr}[1]{\color{mythistle}{#1}}


%---------------- Abbreviations ------------------------------------

\newcommand{\bl}{\begin{itemize}}
\newcommand{\el}{\end{itemize}}
\newcommand{\be}{\begin{enumerate}}
\newcommand{\ee}{\end{enumerate}}
\newcommand{\ii}{\item}
\newcommand{\bea}{\begin{eqnarray*}}
\newcommand{\eea}{\end{eqnarray*}}
\newcommand{\trace}{\mbox{trace}}
\newcommand{\rank}{\mbox{rank}}
\newcommand{\diag}{\mbox{diag}}

\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}

\newcommand{\bmx}{\left[ \begin{array}}
\newcommand{\emx}{\end{array} \right]}

\def\website{{\tt www.mysite}}
\def\Blas{{\sc Blas}}
\def\Fortran{{\sc Fortran}}
\def\Lapack{{\sc Lapack}}
\def\Maple{{\sc Maple}}
\def\Matlab{{MATLAB}}
\def\Netlib{{\sc Netlib}}
\def\bicg{{\sc bi-cg}}
\def\bvp{{\sc bvp}}
\def\bvps{{\sc bvp}s}
\def\cg{{\sc cg}}
\def\cgs{{\sc cgs}}
\def\dae{{\sc dae}}
\def\daes{{\sc dae}s}
\def\dde{{\sc dde}}
\def\ddes{{\sc dde}s}
\def\gmres{{\sc gmres}}
\def\ivp{{\sc ivp}}
\def\ivps{{\sc ivp}s}
\def\lsqr{{\sc lsqr}}
\def\mr{{\sc mr}}
\def\ode{{\sc ode}}
\def\odes{{\sc ode}s}
\def\pcg{{\sc pcg}}
\def\qmr{{\sc qmr}}
\def\sim{{\sc sim}}
\def\sor{{\sc sor}}
\def\symmlq{{\sc symmlq}}
\def\half{\frac{1}{2}}
\def\flip{\hat{\bf{x}}^c}

\def\deriv{{\rm d}}

%---------------- Superscripts -------------------------------------

\newcommand{\inv}{\/^{-1}}
\newcommand{\kk}{^{(k)}}
\newcommand{\jj}{^{(j)}}
\newcommand{\zz}{^{(0)}}
\newcommand{\oo}{^{(1)}}
\newcommand{\tw}{^{(2)}}
\newcommand{\kp}{{^{(k+1)}}}
\newcommand{\np}{{^{(n+1)}}}
\newcommand{\kn}{{^{(k+n)}}}

%---------------- Typeface -----------------------------------------

\newcommand{\wantverbatim}[1]{#1}
%\renewcommand{\script}[1]{{\cal{#1}}}
%   \newcommand{\mybf}{\mathbf }
\newcommand{\mybf}[1]{\textbf{\em #1} }
\newcommand{\ud}{\mathrm{d}}


\def\bfa{{\mybf{a}}}
\def\bfb{{\mybf{b}}}
\def\bfbstar{{\mybf{b}_{opt}}}
\def\bfc{{\mybf{c}}}
\def\bfd{{\mybf{d}}}
\def\bfe{{\mybf{e}}}
\def\bff{{\mybf{f}\,}}
\def\bfg{{\mybf{g}}}
\def\bfh{{\mybf{h}}}
\def\bfk{{\mybf{k}}}
\def\bfell{{\bm{\ell}}}
\def\bfm{{\mybf{m}}}
\def\bfn{{\mybf{n}}}
\def\bfp{{\mybf{p}}}
\def\bfpstar{{\mybf{p}_{opt}}}
\def\bfq{{\mybf{q}}}
\def\bfr{{\mybf{r}}}
\def\bfs{{\mybf{s}}}
\def\bft{{\mybf{t}}}
\def\bfu{{\mybf{u}}}
\def\bfv{{\mybf{v}}}
\def\bfw{{\mybf{w}}}
\def\bfx{{\mybf{x}}}
\def\bfxparticular{{\mybf{x}_{good}}}
\def\bfyparticular{{\mybf{y}_{good}}}
\def\bfxstar{{\mybf{x}_{opt}}}
\def\bfy{{\mybf{y}}}
\def\bfystar{{\mybf{y}_{opt}}}
\def\bfz{{\mybf{z}}}
\def\bfzed{{\bf{0}}}
\def\bfone{{\bf{1}}}
\def\bfxexact{{\widehat{\bfx}}}
\def\xexact{{\hat{x}}}
\newcommand{\bfhae}{{\widehat{\mybf{e}}}}

\def\bfxz{{\mybf{x}^{(0)}}}
\def\bfxk{{\mybf{x}^{(k)}}}
\def\bfxkp{{\mybf{x}^{(k+1)}}}
\def\xkpi{{x}_i^{(k+1)}}
\def\xkhi{{x}_i^{(k+1/2)}}
\def\xkpj{{x}_j^{(k+1)}}
\def\xkhj{{x}_j^{(k+1/2)}}
\def\xkj{{x}_j^{(k)}}
\def\bfuk{{\mybf{u}^{(k)}}}
\def\bfukp{{\mybf{u}^{(k+1)}}}
\def\bfuz{{\mybf{u}^{(0)}}}
\def\ukpi{u^{(k+1)}_i}
\def\ukpj{u^{(k+1)}_j}
\def\ukj{u^{(k)}_j}

\def\bfA{{\mybf{A}}}
\def\bfB{{\mybf{B}}}
\def\bfC{{\mybf{C}}}
\def\bfD{{\mybf{D}}}
\def\bfE{{\mybf{E}}}
\def\bfF{{\mybf{F}}}
\def\bfG{{\mybf{G}}}
\def\bfGhat{{\widehat{\mybf{G}}}}
\def\bfH{{\mybf{H}}}
\newcommand{\bfHa}{{\mybf{B}}} % approximation to Hessian
\newcommand{\bfHainv}{{\mybf{C}}} % approximation to Hessian inverse
\def\bfI{{\mybf{I}}}
\def\bfJ{{\mybf{J}}}
\def\bfK{{\mybf{K}}}
\def\bfL{{\mybf{L}}}
\def\bfM{{\mybf{M}}}
\def\bfN{{\mybf{N}}}
\def\bfP{{\mybf{P}}}
\def\bfQ{{\mybf{Q}}}
\def\bfR{{\mybf{R}}}
\def\bfS{{\mybf{S}}}
\def\bfT{{\mybf{T}}}
\def\bfU{{\mybf{U}}}
\def\bfV{{\mybf{V}}}
\def\bfW{{\mybf{W}}}
\def\bfX{{\mybf{X}}}
\def\bfY{{\mybf{Y}}}
\def\bfZ{{\mybf{Z}}}
\def\bfDelta{\bm{\Delta}}
\def\bfLambda{\bm{\Lambda}}
\def\bfSigma{\bm{\Sigma}}
\def\bfPhi{\bm{\Phi}}

\def\bfalpha{\bm{\alpha}}
\def\bfdelta{\bm{\delta}}
\def\bflambda{\bm{\lambda}}
\def\bftheta{\bm{\theta}}
\def\bfeta{\bm{\eta}}
\def\bfeps{\bm{\epsilon}}
\def\bfgamma{\bm{\gamma}}
\def\bfrho{\bm{\rho}}
\def\bfsigma{\bm{\sigma}}

%------------------ Other ----------------------

\newcommand{\Omegabar}{\bar{\Omega}}
\newcommand{\grad}{\bigtriangledown}
\newcommand{\innerprod}[1]{\langle {#1} \rangle}
\newcommand{\homepage}{
\begin{quote}
{\tt www.cs.umd.edu/users/oleary/SCCS/}
\end{quote}
}



